An Introduction to Liquid Haskell

This paper is a tutorial introducing the underlying technology and the use of the tool Liquid Haskell, a type-checker for the functional language Haskell that can help programmers to verify non-trivial properties of their programs with a low effort. The first sections introduce the technology of Liquid Types by explaining its principles and summarizing how its type inference algorithm manages to prove properties. The remaining sections present a selection of Haskell examples and show the kind of properties that can be proved with the system.

==> eptcsdata.tex <==
\providecommand{\firstpage}{68}
\providecommand{\publicationstatus}{A. Villanueva (Ed.): PROLE 2016\\
EPTCS 237, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.237.5}{10.4204/EPTCS.237.5}}
\pdfoutput=1

